Asynchronous Functional Sessions: Cyclic and Concurrent

We present Concurrent GV (CGV), a functional calculus with message-passing concurrency governed by session types. With respect to prior calculi, CGV has increased support for concurrent evaluation and for cyclic network topologies. The design of CGV draws on APCP, a session-typed asynchronous pi-calculus developed in prior work. Technical contributions are (i) the syntax, semantics, and type system of CGV; (ii) a correct translation of CGV into APCP; (iii) a technique for establishing deadlock-free CGV programs, by resorting to APCP's priority-based type system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{75}
\providecommand{\publicationstatus}{V. Castiglioni and C. A. Mezzina (Eds): Combined Workshop on \\ Expressiveness in Concurrency and Structural Operational Semantics 2022 \\ (EXPRESS/SOS 2022).\\
EPTCS 368, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.368.5}{10.4204/EPTCS.368.5}}

